Multiple-beam Interference Spectroscopy: Instrument Analysis and Spectrum Reconstruction

Hyperspectral imaging systems based on multiple-beam interference (MBI), such as Fabry-Perot interferometry, are attracting interest due to their compact design, high throughput, and fine resolution. Unlike dispersive devices, which measure spectra directly, the desired spectra in interferometric systems are reconstructed from measured interferograms. Although the response of MBI devices is modeled by the Airy function, existing reconstruction techniques are often limited to Fourier-transform spectroscopy, which is tailored for two-beam interference (TBI). These methods impose limitations for MBI and are susceptible to non-idealities like irregular sampling and noise, highlighting the need for an in-depth numerical framework. To fill this gap, we propose a rigorous taxonomy of the TBI and MBI instrument description and propose a unified Bayesian formulation which both embeds the description of existing literature works and adds some of the real-world non-idealities of the acquisition process. Under this framework, we provide a comprehensive review of spectroscopy forward and inverse models. In the forward model, we propose a thorough analysis of the discretization of the continuous model and the ill-posedness of the problem. In the inverse model, we extend the range of existing solutions for spectrum reconstruction, framing them as an optimization problem. Specifically, we provide a progressive comparative analysis of reconstruction methods from more specific to more general scenarios, up to employing the proposed Bayesian framework with prior knowledge, such as sparsity constraints. Experiments on simulated and real data demonstrate the framework's flexibility and noise robustness. The code is available at https://github.com/mhmdjouni/inverspyctrometry.

==> refs_backup.tex <==
@article{MongLE21:spm,
	title={Algorithm unrolling: Interpretable, efficient deep learning for signal and image processing},
	author={Monga, Vishal and Li, Yuelong and Eldar, Yonina C},
	journal={IEEE Signal Processing Magazine},
	volume={38},
	number={2},
	pages={18--44},
	year={2021},
	publisher={IEEE}
}

@book{Idie13:book,
	title={Bayesian approach to inverse problems},
	author={Idier, J{\'e}r{\^o}me},
	year={2013},
	publisher={John Wiley \& Sons}
}

@article{LoriV11:ip,
	title={On a generalization of the iterative soft-thresholding algorithm for the case of non-separable penalty},
	author={Loris, Ignace and Verhoeven, Caroline},
	journal={Inverse Problems},
	volume={27},
	number={12},
	pages={125007},
	year={2011},
	publisher={IOP Publishing}
}

@article{Hans90:jssc,
	title={Truncated singular value decomposition solutions to discrete ill-posed problems with ill-determined numerical rank},
	author={Hansen, Per Christian},
	journal={SIAM Journal on Scientific and Statistical Computing},
	volume={11},
	number={3},
	pages={503--518},
	year={1990},
	publisher={SIAM}
}

@article{GoluHO99:jmaa,
	title={Tikhonov regularization and total least squares},
	author={Golub, Gene H and Hansen, Per Christian and O'Leary, Dianne P},
	journal={SIAM journal on matrix analysis and applications},
	volume={21},
	number={1},
	pages={185--194},
	year={1999},
	publisher={SIAM}
}

@article{PariB14:fto,
	title={Proximal algorithms},
	author={Parikh, Neal and Boyd, Stephen and others},
	journal={Foundations and trends{\textregistered} in Optimization},
	volume={1},
	number={3},
	pages={127--239},
	year={2014},
	publisher={Now Publishers, Inc.}
}

@article{DuraMSC16:jis,
	title={Collaborative total variation: a general framework for vectorial TV models},
	author={Duran, Joan and Moeller, Michael and Sbert, Catalina and Cremers, Daniel},
	journal={SIAM Journal on Imaging Sciences},
	volume={9},
	number={1},
	pages={116--151},
	year={2016},
	publisher={SIAM}
}

@article{DiamSHW17:arxiv,
	title={Unrolled optimization with deep priors},
	author={Diamond, Steven and Sitzmann, Vincent and Heide, Felix and Wetzstein, Gordon},
	journal={arXiv preprint arXiv:1705.08041},
	year={2017}
}

@article{ZhanLZZVT21:tpami,
	title={Plug-and-play image restoration with deep denoiser prior},
	author={Zhang, Kai and Li, Yawei and Zuo, Wangmeng and Zhang, Lei and Van Gool, Luc and Timofte, Radu},
	journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
	year={2021},
	publisher={IEEE}
}

@inproceedings{GousPLRVCFD22:igarss,
	title={ImSPOC: A Novel Compact Hyperspectral Camera for the Monitoring of Atmospheric Gases},
	author={Gousset, S and Picone, D and Le Coarer, E and Rodrigo, JM and Voisin, D and Croize, L and Ferrec, Y and Dalla Mura, M},
	booktitle={IGARSS 2022-2022 IEEE International Geoscience and Remote Sensing Symposium},
	pages={5293--5296},
	year={2022},
	organization={IEEE}
}

@article{CondKCH19:arxiv,
	title={Proximal splitting algorithms for convex optimization: A tour of recent advances, with new twists},
	author={Condat, Laurent and Kitahara, Daichi and Contreras, Andr{\'e}s and Hirabayashi, Akira},
	journal={arXiv e-prints},
	pages={arXiv--1912},
	year={2019}
}


@Book{Eism12,
	author    = {Eismann, Michael T.},
	publisher = {Society of Photo-Optical Instrumentation Engineers},
	title     = {Hyperspectral remote sensing},
	year      = {2012},
	isbn      = {9780819487872},
	series    = {Press Monographs},
	lccn      = {2011046489},
}

@Book{Mano16,
	author    = {Manolakis, Dimitris and Lockwood, Ronald and Cooley, Thomas},
	publisher = {Cambridge University Press},
	title     = {Hyperspectral imaging remote sensing: physics, sensors, and algorithms},
	year      = {2016},
	isbn      = {9781107083660},
	pages     = {706},
}


@Book{Dona19,
	editor    = {Marco Donatelli and Stefano Serra-Capizzano},
	publisher = {Springer-Verlag GmbH},
	title     = {Computational methods for inverse problems in imaging},
	year      = {2019},
	date      = {2019-11-26},
	ean       = {9783030328825},
	file      = {:Dona19 - Computational Methods for Inverse Problems in Imaging.pdf:PDF},
	groups    = {Inversion},
	pagetotal = {166},
	url       = {https://www.ebook.de/de/product/38436013/computational_methods_for_inverse_problems_in_imaging.html},
}

@Article{oiknine-2018-multi-apert,
	author       = {Yaniv Oiknine and Isaac August and Adrian Stern},
	title	       = {Multi-Aperture Snapshot Compressive Hyperspectral Camera},
	journal      = {Opt. Lett.},
	year	       = 2018,
	volume       = 43,
	number       = 20,
	pages	       = {5042-5045},
	month	       = {Oct},
	keywords     = {Emission; Lens arrays; Optical depth; Reconstruction algorithms; Spatial resolution; Spectral imaging},
	doi	       = {10.1364/OL.43.005042},
	url	       = {https://opg.optica.org/ol/abstract.cfm?URI=ol-43-20-5042},
	publisher    = {Optica Publishing Group}
}

@Article{oiknine-2018-nir-hyper,
	author       = {Yaniv Oiknine and Isaac August and Dan G Blumberg and Adrian Stern},
	title	       = {Nir Hyperspectral Compressive Imager Based on a Modified Fabry-Perot Resonator},
	journal      = {Journal of Optics},
	year	       = 2018,
	volume       = 20,
	number       = 4,
	pages	       = 044011,
	month	       = {mar},
	doi	       = {10.1088/2040-8986/aab3b8},
	url	       = {https://dx.doi.org/10.1088/2040-8986/aab3b8},
	publisher    = {IOP Publishing}
}

@Article{zucco-2014-fabry-perot,
	author       = {Zucco, Massimo and Pisani, Marco and Caricato, Valentina and Egidi, Andrea},
	title	       = {A hyperspectral imager based on a Fabry-Perot interferometer with dielectric mirrors},
	journal      = {Optics express},
	year	       = 2014,
	volume       = 22,
	number       = 2,
	pages	       = {1824-1834},
	publisher    = {Optical Society of America}
}

@Article{PisaZ09:oe,
	author       = {Pisani, Marco and Zucco, Massimo},
	title	       = {Compact imaging spectrometer combining {Fourier} transform spectroscopy with a Fabry-Perot
	interferometer},
	journal      = {Optics express},
	year	       = 2009,
	volume       = 17,
	number       = 10,
	pages	       = {8319-8331},
	publisher    = {Optical Society of America}
}

@Book{Hech16,
	author    = {Eugene Hecht},
	publisher = {Pearson},
	title     = {Optics (5th edition)},
	year      = {2016},
	isbn      = {978-0133977226},
	file      = {:Hech16 - Optics (5th Edition).pdf:PDF},
	groups    = {optics},
	url       = {https://www.amazon.com/Optics-5th-Eugene-Hecht/dp/0133977226?SubscriptionId=0JYN1NVW651KCA56C102&tag=techkie-20&linkCode=xm2&camp=2025&creative=165953&creativeASIN=0133977226}
}

@Book{Hari10,
	author    = {Hariharan, Parameswaran},
	publisher = {Elsevier},
	title     = {Basics of interferometry},
	year      = {2010},
	file      = {:Hari10 - Basics of Interferometry.pdf:PDF},
	groups    = {imSPOC},
}

@Book{Hari03,
	author    = {Hariharan, Parameswaran},
	publisher = {Elsevier},
	title     = {Optical interferometry, 2e},
	year      = {2003},
	file      = {:Hari03 - Optical Interferometry, 2e.pdf:PDF},
	groups    = {imSPOC},
}

@inproceedings{JounPD23:icassp,
	title={Model-based spectral reconstruction of interferometric acquisitions},
	author={Jouni, Mohamad and Picone, Daniele and Dalla Mura, Mauro},
	booktitle={ICASSP 2023-2023 IEEE International Conference on Acoustics, Speech, and Signal Processing},
	pages={},
	year={2023},
	organization={IEEE}
}

@article{BeckT09:jis,
  title={A fast iterative shrinkage-thresholding algorithm for linear inverse problems},
  author={Beck, Amir and Teboulle, Marc},
  journal={SIAM journal on imaging sciences},
  volume={2},
  number={1},
  pages={183--202},
  year={2009},
  publisher={SIAM}
}

@article{HamiBS15:cl,
  title={Signal bandwidth impact on maximum-minimum eigenvalue detection},
  author={Hamid, Mohamed and Bj{\"o}rsell, Niclas and Slimane, Slimane Ben},
  journal={IEEE Communications Letters},
  volume={19},
  number={3},
  pages={395--398},
  year={2015},
  publisher={IEEE}
}

@Article{CondKCH23:siam,
	author    = {Condat, Laurent and Kitahara, Daichi and Contreras, Andr{\'e}s and Hirabayashi, Akira},
	journal   = {SIAM Review},
	title     = {Proximal splitting algorithms for convex optimization: A tour of recent advances, with new twists},
	year      = {2023},
	month     = {may},
	number    = {2},
	pages     = {375--435},
	volume    = {65},
	doi       = {10.1137/20m1379344},
	file      = {:Cond22 - Proximal Splitting Algorithms_ a Tour of Recent Advances, with New Twists.pdf:PDF},
	groups    = {optimization},
	publisher = {Society for Industrial {\&} Applied Mathematics ({SIAM})},
}

@article{PicoGDFL23:oe,
	title={Interferometer response characterization algorithm for multi-aperture Fabry-Perot imaging spectrometers},
	author={Picone, Daniele and Gousset, Silv{\`e}re and Dalla Mura, Mauro and Ferrec, Yann and le Coarer, Etienne},
	journal={Optics Express},
	volume={31},
	number={14},
	pages={23066--23085},
	year={2023},
	publisher={Optica Publishing Group}
}

@article{BrisSBDRGF04:ao,
	title={Spectrogonio radiometer for the study of the bidirectional reflectance and polarization functions of planetary surfaces. 1. Design and tests},
	author={Brissaud, Olivier and Schmitt, Bernard and Bonnefoy, Nicolas and Doute, Sylvain and Rabou, Patrick and Grundy, Will and Fily, Michel},
	journal={Applied Optics},
	volume={43},
	number={9},
	pages={1926--1937},
	year={2004},
	publisher={Optica Publishing Group}
}

@misc{SpecimIQ,
	author={{Specim, Spectral Imaging Ltd}},
	title={Specim {IQ} {H}yperspectral {G}oes {M}obile},
	howpublished={
		Specim IQ.
		\url{https://www.specim.com/iq/}
		(accessed Oct. 4, 2023).
	},
}

@misc{CalibriteCC,
	author={Calibrite},
	title={Color{C}hecker {C}lassic},
	howpublished={
	ColorChecker Classic.
	\url{https://calibrite.com/us/product/colorchecker-classic/}
	(accessed Oct. 4, 2023).
	},
}

@Misc{GuerLFD18:imspoc,
	author      = {Guerineau, Nicolas and Le Coarer, Etienne and Ferrec, Yann and De La Barriere, Florence},
	month       = jan,
	note        = {{FR} patent 1,656,162},
	title       = {{Fourier} transform multi-channel spectral imager},
	year        = {2018},
	day         = {04},
	dayfiled    = {30},
	groups      = {imspoc},
	language    = {French, English},
	monthfiled  = {#jun#},
	nationality = {FR},
	number      = {WO2018002558A1},
	url         = {https://patents.google.com/patent/WO2018002558A1/fr},
	yearfiled   = {2016},
}

@ARTICLE{ZuccCEP15:tim,
	
	author={Zucco, Massimo and Caricato, Valentina and Egidi, Andrea and Pisani, Marco},
	
	journal={IEEE Transactions on Instrumentation and Measurement}, 
	
	title={A Hyperspectral Camera in the UVA Band}, 
	
	year={2015},
	
	volume={64},
	
	number={6},
	
	pages={1425-1430},
	
	doi={10.1109/TIM.2014.2381751}
}

@phdthesis{Caro12:thesis,
	title={Irregular sampling restoration. Theory and applications to satellite images and signals.},
	author={Julien, Caron},
	year={2012},
	school={Universit{\'e} de Picardie Jules Verne}
}

@book{BoydV04:book,
	title={Convex optimization},
	author={Boyd, Stephen P and Vandenberghe, Lieven},
	year={2004},
	publisher={Cambridge university press}
}

@book{BornW13:book,
	title={Principles of optics: electromagnetic theory of propagation, interference and diffraction of light},
	author={Born, Max and Wolf, Emil},
	year={2013},
	publisher={Elsevier}
}

@article{SheiN23:arxiv,
	title={Theory and Instrumentation of {Fourier} Transform Spectroscopy},
	author={Sheikh-Sofla, Sohrab and Neshat, Mohammad},
	journal={arXiv preprint arXiv:2302.00086},
	year={2023}
}

@book{Cars21:book,
	title={Introduction to the Theory of {Fourier}'s Series and Integrals},
	author={Carslaw, Horatio Scott},
	volume={1},
	year={1921},
	publisher={Macmillan and Company, limited}
}

@misc{mhmdjouni:inverspyctrometry,
	author       = {mhmdjouni},
	title        = {inverspyctrometry},
	howpublished = "\url{https://github.com/mhmdjouni/inverspyctrometry}",
	year         = {2024},
}

@misc{mhmdjouni:dataset,
	author       = {mhmdjouni},
	title        = {datasetName},
	howpublished = "\url{https://huggingface.co/mhmdjouni/datasetname}",
	year         = {2024},
}

@article{Bell73:book,
	title={Introductory {Fourier} transform spectroscopy},
	author={Bell, Robert John},
	journal={American Journal of Physics},
	volume={41},
	number={1},
	pages={149--151},
	year={1973},
	publisher={American Association of Physics Teachers}
}

@book{Hern88:book,
	title={Fabry-perot interferometers},
	author={Hern{\'a}ndez, Gonzalo},
	number={3},
	year={1988},
	publisher={Cambridge University Press}
}

@article{AhmeNR74:tc,
	title={Discrete cosine transform},
	author={Ahmed, Nasir and Natarajan, T\_ and Rao, Kamisetty R},
	journal={IEEE transactions on Computers},
	volume={100},
	number={1},
	pages={90--93},
	year={1974},
	publisher={IEEE}
}

@book{Hans10:book,
        author = {Hansen, Per Christian},
        title = {Discrete inverse problems: insight and algorithms},
        publisher = {SIAM},
        year = {2010},
}


      @Article{conde-2002-deriv-wavel,
        author = {Conde, Mark},
        title = {Deriving Wavelength Spectra From Fringe Images From a Fixed-Gap Single-Etalon Fabry-Perot Spectrometer},
        journal = {Applied Optics},
        year = {2002},
        volume = {41},
        number = {14},
        pages = {2672},
        month = {May},
        doi = {10.1364/ao.41.002672},
        url = {http://dx.doi.org/10.1364/AO.41.002672},
        issn = {1539-4522},
        publisher = {Optica Publishing Group}
      }

      @Article{okada-1989-infor-proces-spect,
        author = {Okada, Katsuhiko and Ishibashi, Yoshihiro and Kitade, Atsuo},
        title = {Information Processing in Spectroscopy},
        journal = {Applied Optics},
        year = 1989,
        volume = {28},
        number = {8},
        pages = {1546},
        month = {Apr},
        doi = {10.1364/ao.28.001546},
        url = {http://dx.doi.org/10.1364/AO.28.001546},
        issn = {1539-4522},
        publisher = {Optica Publishing Group}
      }

      @Article{zipoy-1979-fabry-perot,
        author = {Zipoy, David M.},
        title = {Fabry-Perot Inversion Algorithm},
        journal = {Applied Optics},
        year = 1979,
        volume = {18},
        number = {12},
        pages = {1988},
        month = {Jun},
        doi = {10.1364/ao.18.001988},
        url = {http://dx.doi.org/10.1364/AO.18.001988},
        issn = {1539-4522},
        publisher = {Optica Publishing Group}
      }

      @Article{cooper-1971-analy-fabry,
        author = {Cooper, V. G.},
        title = {Analysis of Fabry-Perot Interferograms By Means of Their {Fourier} Transforms},
        journal = {Applied Optics},
        year = 1971,
        volume = {10},
        number = {3},
        pages = {525},
        month = {Mar},
        doi = {10.1364/ao.10.000525},
        url = {http://dx.doi.org/10.1364/AO.10.000525},
        issn = {1539-4522},
        publisher = {Optica Publishing Group}
      }

@article{reardon-2008-charac-fabry,
  title={Characterization of Fabry-Perot interferometers and multi-etalon transmission profiles-The IBIS instrumental profile},
  author={Reardon, KP and Cavallini, F},
  journal={Astronomy \& Astrophysics},
  volume={481},
  number={3},
  pages={897--912},
  year={2008},
  publisher={EDP Sciences}
}

      @Article{koo-1987-decon-algor,
        author = {Koo, Ja-Yong and Kim, Jong-Jean},
        title = {Deconvolution Algorithm for a Fabry-Perot Interferometer},
        journal = {Applied Optics},
        year = 1987,
        volume = {26},
        number = {6},
        pages = {1094},
        month = {Mar},
        doi = {10.1364/ao.26.001094},
        url = {http://dx.doi.org/10.1364/AO.26.001094},
        issn = {1539-4522},
        publisher = {Optica Publishing Group}
      }

      @Article{elzeiny-2021-compl-kernel,
        author = {ElZeiny, Walid ElSayed and Sabry, Yasser M. and Khalil, Diaa A.},
        title = {Complex Kernel-Based Spectrum Reconstruction Algorithm for Cascaded Fabry-Perot Interferometric Spectrometer},
        journal = {Applied Optics},
        year = 2021,
        volume = {60},
        number = {29},
        pages = {8999},
        month = {Oct},
        doi = {10.1364/ao.433417},
        url = {http://dx.doi.org/10.1364/AO.433417},
        issn = {2155-3165},
        publisher = {Optica Publishing Group}
      }

      @Article{yang-2020-theor-analy,
        author = {Yang, Qinghua},
        title = {Theoretical Analysis of Compact Ultrahigh-Spectral-Resolution Infrared Imaging Spectrometer},
        journal = {Optics Express},
        year = 2020,
        volume = {28},
        number = {11},
        pages = {16616},
        month = {May},
        doi = {10.1364/oe.395475},
        url = {http://dx.doi.org/10.1364/OE.395475},
        issn = {1094-4087},
        publisher = {Optica Publishing Group}
      }

@article{yang-2019-compac-ultrah,
  title={Compact ultrahigh resolution interferometric spectrometer},
  author={Yang, Qinghua},
  journal={Optics Express},
  volume={27},
  number={21},
  pages={30606--30617},
  year={2019},
  publisher={Optica Publishing Group}
}

      @Article{el-sayed-2018-trans-algor,
        author = {El-Sayed, Islam Samir and Sabry, Yasser M. and ElZeiny, Walid ElSayd and Badra, Niveen and Khalil, Diaa A.},
        title = {Transformation Algorithm and Analysis of the {Fourier} Transform Spectrometer Based on Cascaded Fabry-Perot Interferometers},
        journal = {Applied Optics},
        year = 2018,
        volume = {57},
        number = {25},
        pages = {7225},
        month = {Aug},
        doi = {10.1364/ao.57.007225},
        url = {http://dx.doi.org/10.1364/AO.57.007225},
        issn = {2155-3165},
        publisher = {The Optical Society}
      }

      @Article{yang-2020-first-order,
        author = {Yang, Qinghua},
        title = {First Order Design of Compact, Broadband, High Spectral Resolution Ultraviolet-Visible Imaging Spectrometer},
        journal = {Optics Express},
        year = 2020,
        volume = {28},
        number = {4},
        pages = {5587},
        month = {Feb},
        doi = {10.1364/oe.384603},
        url = {http://dx.doi.org/10.1364/OE.384603},
        issn = {1094-4087},
        publisher = {Optica Publishing Group}
      }

@article{xu2018ultra,
  title={Ultra-compact {Fourier} transform imaging spectrometer using a focal plane birefringent interferometer},
  author={Xu, Yixuan and Li, Jianxin and Bai, Caixun and Yuan, Heng and Liu, Jie},
  journal={Optics Letters},
  volume={43},
  number={17},
  pages={4081--4084},
  year={2018},
  publisher={Optica Publishing Group}
}

      @InProceedings{lucey-2014-{Fourier}-fabry,
        author = {Lucey, Paul G. and Akagi, Jason and Bingham, Adam L. and Hinrichs, John L. and Knobbe, Edward T.},
        title = {A compact {Fourier} transform imaging spectrometer employing a variable gap Fabry-Perot interferometer},
        booktitle = {Next-Generation Spectroscopic Technologies VII},
        year = {2014},
        editor = {Druy, Mark A. and Crocombe, Richard A.},
        month = {May},
        publisher = {SPIE},
        doi = {10.1117/12.2050826},
        url = {http://dx.doi.org/10.1117/12.2050826},
        ISSN = {0277-786X}
      }

@inproceedings{wright-2022-hyti,
    title={HYTI: High Spectral Resolution Thermal Imaging from a Cubesat},
    author={Wright, Robert and Nunes, Miguel and Lucey, Paul and Gunapala, Sarath and Ting, David and Ferrari-Wong, Chiara and Flynn, Luke and Soibel, Alexander and others},
    booktitle={IGARSS 2022-2022 IEEE International Geoscience and Remote Sensing Symposium},
    pages={7143--7145},
    year={2022},
    organization={IEEE}
}

@inproceedings{wright-2023-hyti,
    title={The HyTI mission},
    author={Wright, Robert and Nunes, Miguel A and Lucey, Paul G and Gunapala, Sarath and Ting, David and Ferrari-Wong, Chiara and Flynn, Luke P and George, Tom and others},
    booktitle={Sensors, Systems, and Next-Generation Satellites XXVII},
    volume={12729},
    pages={6--9},
    year={2023},
    organization={SPIE}
}

@Article{chen-2006-simpl-terah,
    author = {Chen, Li-Jin and Kao, Tzeng-Fu and Lu, Ja-Yu and Sun, Chi-Kuang},
    title = {A Simple Terahertz Spectrometer Based on a Low-Reflectivity Fabry-Perot Interferometer Using {Fourier} Transform Spectroscopy},
    journal = {Optics Express},
    year = {2006},
    volume = {14},
    number = {9},
    pages = {3840},
    doi = {10.1364/oe.14.003840},
    url = {http://dx.doi.org/10.1364/OE.14.003840},
    issn = {1094-4087},
    publisher = {Optica Publishing Group}
}

@Article{jovanov-2011-trans-{Fourier},
    author = {Jovanov, Vladislav and Bunte, Eerke and Stiebig, Helmut and Knipp, Dietmar},
    title = {Transparent {Fourier} Transform Spectrometer},
    journal = {Optics Letters},
    year = 2011,
    volume = 36,
    number = 2,
    pages = 274,
    month = {Jan},
    doi = {10.1364/ol.36.000274},
    url = {http://dx.doi.org/10.1364/OL.36.000274},
    issn = {1539-4794},
    publisher = {The Optical Society}
}

@Article{al-saeed-2016-{Fourier}-trans,
      author = {Tarek A. Al-Saeed and Diaa A. Khalil},
      title = {{Fourier} Transform Spectrometer Based on {Fabry}{\textendash}{Perot} Interferometer},
      journal = {Applied Optics},
      year = 2016,
      volume = 55,
      number = 20,
      pages = 5322,
      month = jul,
      file = {/home/dallamum/work/research/biblio/pdfs/articles/al-saeed-2016-{Fourier}-trans.pdf},
      doi = {10.1364/ao.55.005322},
      publisher = {The Optical Society}
}

@InProceedings{pisani-2017-high,
      author = {Pisani, M. and Bianco, P. and Zucco, M.},
      title = {High throughput, compact imaging spectrometer},
      booktitle = {International Conference on Space Optics - ICSO 2010},
      year = 2017,
      editor = {Kadowaki, Naoto},
      month = nov,
      publisher = {SPIE},
      doi = {10.1117/12.2309244},
      url = {http://dx.doi.org/10.1117/12.2309244}
}

@article{eskelinen-2019-comput-method,
  title={Computational methods for hyperspectral imaging using Fabry--Perot interferometers and colour cameras},
  author={Eskelinen, Matti},
  journal={JYU dissertations},
  year={2019}
}

      @InProceedings{crites-2015-therm-infrar,
      author = {Crites, S. T. and Wright, R. and Lucey, P. G. and Chan, J. and Gabrieli, A. and Garbeil, H. and
      Horton, K. A. and Imai-Hong, A. K. R. and Pilger, E. J. and Wood, M. and Yoneshige, L.},
      title = {The Thermal Infrared Compact Imaging Spectrometer (TIRCIS): a follow-on to the Space Ultra Compact
      Hyperspectral Imager (SUCHI)},
      booktitle = {Sensors and Systems for Space Applications VIII},
      year = 2015,
      editor = {Pham, Khanh D. and Chen, Genshe},
      month = may,
      publisher = {SPIE},
      doi = {10.1117/12.2185649},
      url = {http://dx.doi.org/10.1117/12.2185649},
      ISSN = {0277-786X}
      }

@PhdThesis{pola-2016-miniat,
    author = {Pola Fossi, Armande},
    title = {{Miniaturisation d'une cam{\'e}ra hyperspectrale infrarouge}},
    school = {{Universit{\'e} Paris Saclay (COmUE)}},
    year = 2016,
    type = {Theses},
    month = Dec,
    keywords = {Remote sensing ; Birefringent interferometer ; Compact ; Hyperspectral imaging ; Infrared ; Camera ;
    Camera ; Infrarouge ; Imagerie hyperspectrale ; Compact ; Interferometre birefringent ;
    T{\'e}l{\'e}detection},
    HAL_ID = {tel-01511621},
    HAL_VERSION = {v1},
    NUMBER = {2016SACLS568},
    PDF = {https://theses.hal.science/tel-01511621/file/75700_POLAFOSSI_2016_diffusion.pdf},
    URL = {https://theses.hal.science/tel-01511621}
}

@book{nikolic-2011-{Fourier}-trans,
  title={{Fourier} transforms: New analytical approaches and FTIR strategies},
  author={Nikolic, Goran},
  year={2011},
  publisher={BoD--Books on Demand}
}

@article{yoshihara1979far,
  title={Far infra-red spectroscopy by the Fabry-Perot interferometer},
  author={Yoshihara, Kunio and Kitade, Atsuo},
  journal={Optica Acta: International Journal of Optics},
  volume={26},
  number={8},
  pages={1049--1056},
  year={1979},
  publisher={Taylor \& Francis}
}

@article{jacquinot1954luminosity,
  title={The luminosity of spectrometers with prisms, gratings, or Fabry-Perot etalons},
  author={Jacquinot, Pierre},
  journal={JOSA},
  volume={44},
  number={10},
  pages={761--765},
  year={1954},
  publisher={Optica Publishing Group}
}

@article{fellgett2006nature,
  title={The nature and origin of multiplex {Fourier} spectrometry},
  author={Fellgett, PB},
  journal={Notes and Records of the Royal Society},
  volume={60},
  number={1},
  pages={91--93},
  year={2006},
  publisher={The Royal Society London}
}

@article{wang2010comparison,
  title={The comparison of environmental effects on Michelson and Fabry-Perot interferometers utilized for the displacement measurement},
  author={Wang, Yung-Cheng and Shyu, Lih-Horng and Chang, Chung-Ping},
  journal={Sensors},
  volume={10},
  number={4},
  pages={2577--2586},
  year={2010},
  publisher={Molecular Diversity Preservation International (MDPI)}
}

@article{alcock2006compact,
  title={A compact, high numerical aperture imaging {Fourier} transform spectrometer and its application},
  author={Alcock, RD and Coupland, JM},
  journal={Measurement Science and Technology},
  volume={17},
  number={11},
  pages={2861},
  year={2006},
  publisher={IOP Publishing}
}

@article{hays1991multiplex,
  title={Multiplex Fabry--Perot interferometer},
  author={Hays, Paul B and Snell, Hilary E},
  journal={Applied optics},
  volume={30},
  number={22},
  pages={3108--3113},
  year={1991},
  publisher={Optica Publishing Group}
}

@article{cook1995multiplex,
	title={Multiplex Fabry--Perot interferometer: I. Theory},
	author={Cook, William B and Snell, Hilary E and Hays, Paul B},
	journal={Applied optics},
	volume={34},
	number={24},
	pages={5263--5267},
	year={1995},
	publisher={Optica Publishing Group}
}

@article{snell1995multiplex,
  title={Multiplex Fabry--Perot interferometer: II. Laboratory prototype},
  author={Snell, Hilary E and Cook, William B and Hays, Paul B},
  journal={Applied optics},
  volume={34},
  number={24},
  pages={5268--5277},
  year={1995},
  publisher={Optica Publishing Group}
}

@inproceedings{picone2024spectro,
	title={Spectro-spatial hyperspectral image reconstruction from interferometric acquisitions},
	author={Picone, Daniele and Jouni, Mohamad and Dalla Mura, Mauro},
	booktitle={ICASSP 2024-2024 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
	pages={2590--2594},
	year={2024},
	organization={IEEE}
}

@inproceedings{ferrec2023albedo,
	title={Albedo bias reduction for Nanocarb GHG sensor: comparison of panchromatic or hyperspectral ancillary imager, and high finesse or multiple harmonics Fabry-Perot interferometer},
	author={Ferrec, Yann and Croiz{\'e}, Laurence and Foucher, Pierre-Yves},
	booktitle={International Conference on Space Optics—ICSO 2022},
	volume={12777},
	pages={2951--2961},
	year={2023},
	organization={SPIE}
}

@article{tibshirani1996regression,
    title={Regression shrinkage and selection via the lasso},
    author={Tibshirani, Robert},
    journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
    volume={58},
    number={1},
    pages={267--288},
    year={1996},
    publisher={Oxford University Press}
}

